Circuit-Theoretic Joint Parameter-State Estimation of Utility-Scale Photovoltaic, Battery, and Grid Systems

Solar PV and battery storage systems have become integral to modern power grids. Therefore, bulk grid models in real-time operation must include their physical behavior accurately for analysis and optimization. AC state estimation is critical to building real-time bulk power systems models. However, current ACSE techniques do not include detailed physics and measurements for battery and PV systems. This results in sub-optimal estimation results and subsequent less accurate bulk grid models for real-time operation. To address these challenges, we formulate a circuit-theoretic AC state estimator with accurate PV and battery systems physics and corresponding measurements. First, we propose an aggregated equivalent circuit model of the solar PV, battery, and traditional grid components. Next, we add measurements from PV and battery systems to the traditional measurement set to facilitate accurate estimation of the overall grid model. Finally, we develop a circuit-theoretic joint parameter-state estimation algorithm that can accurately estimate grid, PV, and battery system states and is robust against erroneous parameters. To demonstrate the efficacy of the proposed framework, we estimate the states of 10k node transmission networks with hundreds of battery+PV-tied systems. We compare the accuracy against the estimation of stand-alone grid, battery, and PV systems.

==> Nomenclature.tex <==
\section*{Nomenclature}

\addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$V_1,V_2,V_3$}]
%\centering
% \item[$V_1,V_2,V_3$] Three-phase PWM output line voltages.
% \item[$\theta$] Rotor angle (in ``electrical degrees'').
% \item[$\omega$] Rotor (electrical) speed, corresponding to the time derivative of $\theta$.

% \item[Network Components]
\small 
\item[\underline{\textbf{Symbol}}] \underline{\textbf{Interpretation}}\\

\item [\textit{General symbols}]
% \item[$I_r^{kl},I_i^{kl}$] Real/imag c
\item [$\boldsymbol{\mathcal{P}}$] Set of circuit model parameters
\item [$\boldsymbol{\mathcal{P}_\text{U}}$] Set of unknown circuit model parameters
\item  [$\boldsymbol{\mathcal{H}}$] Set of combined network constraints
\item  [$\boldsymbol{\mathcal{Z}}$] Set of measurements
\item[$\boldsymbol{\mathcal{W}}$] Error covariance matrix
\item [$\eta_{inv}$] Inverter efficiency (DC-AC)
\item [$\eta_{rec}$] Rectifier efficiency (AC-DC)
% \item[$\hat{V}_{nk}$] Estimate and true value of $n^{th}$ simulation at $k^{th}$ component
% \item[$\hat{V}_{avg,k}$] Average of estimate at $k^{th}$ component
\item [$\hat{\mathcal{P}}$] Parameter estimates\\

% \item [$\boldsymbol{\mathcal{F}}$]  Set of all components' objectives
% \item  [$N$] Total numbers of simulations run

\item [\textit{Grid specific symbols}]
\item [$\boldsymbol{\mathcal{N}}$] Set of all grid buses
\item [$\boldsymbol{\mathcal{N}_{ZI}}$] Set of zero-injection buses
\item [$\boldsymbol{\mathcal{M}}$] Set of grid measurement circuits (e.g., RTUs measuring injection power)
\item [$\boldsymbol{\mathcal{G}}$] Set of grid components without measurements (e.g., line, transformer, etc.)
\item[$\Tilde{V}_k$] Complex nodal voltage at bus $k$
\item[$V^r_k,V^i_k$] Real/imag voltage at bus $k$
\item[$V^r_{kl},V^i_{kl}$] Real/imag voltage difference between bus $k$ and $l$
% \item[$V^{kl}_r,V^{kl}_i$] Real/imag voltage across bus $k$ and $l$
% \item[$I^r_{L,k},I^i_{L,k}$] Real/imag Load current injection at bus $k$
% \item[$I^r_{fl,jk},I^i_{fl,jk}$] Real/imag current flow between bus $j,k$
\item[$|V|_k,\theta_k$] Voltage magnitude/angle at bus $k$
\item[$P_k,Q_k$] Active/reactive power injection at bus $k$
\item[$\PGk{},\QGk{}$] Real and reactive power injection of generator at bus $k$ 
\item[$\PLk{},\QLk{}$] Real and reactive power injection of load at bus $k$ 
\item[$\Vmagk{}$] Generator regulated voltage magnitude at bus $k$ 
\item[$\Gkz{},\Bkz{}$] Measurement feature transformation terms at bus $k$
% \item [\textbf{z}] Set of measurements
\item[$P_{k,z}, Q_{k,z}$] RTU injection measurements of real/reactive power at bus $k$
\item[$|V|_{k,z}$] RTU injection measurements of volt. mag. at bus $k$
\item[$\ItildG{}, \ItildL{}$] Gen and load complex current injection at bus $k$
\item[$\nrtur{},\nrtui{}$] Real and imag. RTU measurement noise at bus $k$
% \item[$n^k_{|V|}$] Voltage mag. noise term at bus k
\item[$G_{kl},B_{kl}$] Admittance terms between bus $k$ and $l$
\item[$h^{Grid}_{k}$] Set of current-voltage constraints for grid network
physics at bus $k$ 
\\

\item [\textit{PV specific symbols}]%PV
\item [$\boldsymbol{\mathcal{K}}$] Set of bulk grid-connected solar PV
\item[$\RS{},\RSH{}$] Series and shunt resistor of PV ckt
\item[$Z_{Load}$] Grid equivalent impedance seen by the solar PV 
\item [$\VSH{}$] Voltage across on shunt resistor in PV circuit, equal to its open circuit voltage
\item [$\VPV{},\zpvv{}$] Solar PV voltage at the inverter terminal and its measurement
\item[$\VD{}$] Diode voltage in solar PV ckt
\item[$\IPH{},\zphi{}$] PV photocurrent generation and measurement
\item[$\ID{}$] Diode current in PV ckt
\item[$\Izero{}$] Saturation 
current of diode in PV ckt
\item[$\IPV{},\zpvi{}$] Solar PV terminal current and its measurement
% \item[$\ItildPV{}$] PV inverter AC current injection to grid
\item [$P_\text{PV}$] PV DC injection power to inverter
\item[$\npvv{},\npvi{},\nphi{}$] Solar PV voltage, current output, and photocurrent measurement noise terms
\item[$w^\text{PV}_\text{I}, w^\text{PV}_\text{V},w^\text{PV}_\text{PH}$] \; Weights for current, voltage, and photocurrent measurements for PV
\item[$h^{PV}_{k}$] Current-voltage constraints for $k^{th}$ PV ckt on the grid
\\

\item [\textit{Battery specific symbols}]%Battery symbols
\item [$\boldsymbol{\mathcal{L}}$] Set of battery systems connected to bulk grid
\item [$\Vsoc{}$] Voltage representation of battery SOC, range between 0V to 1V for empty to full
\item[$\VOC{}$] Battery open circuit voltage
\item[$\VBatt{},\zbattv{}$] Battery terminal voltage and its measurement
\item[$\IBatt{},\zbatti{}$] DC battery current and its measurement
% \item[$\ItildBatt{}$] battery inverter AC current injection to grid
\item[$\Ccap{}$] Battery equivalent capacitor (F)
\item[$\RSE{},\RSD{}$] Series and self discharge resistor of battery
\item[$h^{\text{Bt}}_{k}$] current-voltage constraints for the $k^{th}$ battery
\item[$\nbattv{},\nbatti{}$] Battery terminal voltage and current measurement noise terms
\item[$w^\text{Bt}_\text{I}, w^\text{Bt}_\text{V}$] Weights for current and voltage measurements for battery




\end{IEEEdescription}

==> Openqestions.tex <==
\begin{itemize}
    \item[1] Try different Norm, e.g. Norm 1 should be robust to bad data measurements
    \item[1.1] The source of bad data can be both form HES or RTU readings, while RTU and HES can be: either BAD, non BAD or both BAD
    \item [1.2] The expectation is to find not only where the bad data is (like Cindy Li's paper) but also show that the HES or the RTU is wrong, so it should be able to show which is wrong or which is more wrong.
    \item [1.3] The unsure part here is the scaling issue will make the RTU one much more impactful compare to HES, so this may not work.
\end{itemize}
